FO-definable transformations of infinite strings

The theory of regular and aperiodic transformations of finite strings has recently received a lot of interest. These classes can be equivalently defined using logic (Monadic second-order logic and first-order logic), two-way machines (regular two-way and aperiodic two-way transducers), and one-way register machines (regular streaming string and aperiodic streaming string transducers). These classes are known to be closed under operations such as sequential composition and regular (star-free) choice; and problems such as functional equivalence and type checking, are decidable for these classes. On the other hand, for infinite strings these results are only known for $\omega$-regular transformations: Alur, Filiot, and Trivedi studied transformations of infinite strings and introduced an extension of streaming string transducers over $\omega$-strings and showed that they capture monadic second-order definable transformations for infinite strings. In this paper we extend their work to recover connection for infinite strings among first-order logic definable transformations, aperiodic two-way transducers, and aperiodic streaming string transducers.

==> sst-fot.tex <==
This section will prove the following theorem in several parts.
\begin{lemma}
\label{lem:sst-fot}
A transformation is FO-definable if it is aperiodic-SST definable.
\end{lemma}
\begin{proof}[Proof (Sketch)]
We show that every aperiodic $1$- bounded SST definable transformation is  definable using FO-transducers.
%We show that for every FO-definable transformation $T$ we can define it using an
%aperiodic $1$-bounded SST. 
A crucial component in the proof of this lemma is to show that the
variable flow in the aperiodic 1-bounded SST is FO-definable.  

%\subsection{FO-definability of variable flow}
%\label{fo:varflow}
%We first show that the variable flow of any aperiodic,1-bounded \sst{} is
%FO-definable. This will be crucial to show that the output predicate $\preceq$ is
%FO-definable.
\begin{proposition}\label{prop:foflow}
    Let $T$ be an aperiodic,1-bounded \sst{} $T$ with set of variables $\varsst$. 
    For all variables $X,Y\in \varsst$, there exists an FO-formula
    $\phi_{X\flows Y}(x,y)$ with two free variables such that,
    for all strings $s\in dom(T)$ and any two positions $i\leq j\in dom(s)$, 
    $s\models \phi_{X\flows Y}(i,j)$ iff $(q_i,X)\flows^{s[i{+}1{:}j]}_1
    (q_j,Y)$, where $q_0\dots q_n \dots$ is the accepting run of $T$ on $s$.
\end{proposition}

Let $X\in\varsst$, $s\in\dom(T)$, $i\in \dom(s)$. Let $P \in 2^Q$ be a Muller accepting set with output $F(P)=X_1 \dots X_n$. Let 
$r = q_0\dots q_{n}\dots$ be an accepting run of $T$ on $s$. Then 
there is a position $j$ such that $\forall k >j$, only states in $P$ are visited. 
On all transitions beyond $j$, $X_1, \dots, X_{n-1}$ remain unchanged, 
while $X_n$ is updated as $X_nu$ for some $u \in (\mathcal{X} \cup \Gamma)^*$.
We say that the pair $(X,i)$ is \emph{useful} if the content of
variable $X$ before reading $s[i]$ will be part of the output after
reading the whole string $s$. 
Formally, for an accepting run $r = q_0\dots q_{j}q_{j+1}\dots$, such that 
only states from the Muller set $P$ are seen after position $j$, we say that
  $(X,i)$ is useful for $s$ if $(q_{i-1}, X)\flows^{s[i{:}j] }_1(q,X_k)$ for some variable $X_k \in F(P)$, $k \leq n$, or 
  if $(q_{i-1}, X)\flows^{s[i{:}\ell] }_1(q,X_n)$, with $q \in P$ and $\ell >j$.  
  Thanks to Proposition \ref{prop:foflow}, this property is FO-definable (Proofs
  of propositions \ref{prop:foflow} and \ref{prop:contribution} are in Appendix \ref{app:varflow}).
%
\begin{proposition}\label{prop:contribution}
    For all $X\in\varsst$, there exists an FO-formula
    $\contribute_X(i)$ s.t. for all strings $s\in dom(T)$ and all
    positions $i\in \dom(s)$, 
    $s\models \contribute_X(i)$ iff $(X,i)$ is useful for string $s$.
\end{proposition}

 %\subsection{SST Output structure} 
%\label{sst-out}
 The output structure for SSTs over finite words has been introduced in \cite{FKT14}. 
It is an intermediate representation of the output, and the transformation of any input string into its   
\sst-output structure will be shown to be FO-definable.
For any \sst{} $T$ and string $s\in\dom(T)$,  the \sst-output structure of $s$ is a relational structure 
$G_T(s)$ obtained by taking, for each variable $X\in\varsst$, two copies of $\dom(s)$, respectively denoted by $X^{in}$ and $X^{out}$.  
For notational convenience we assume that these structures are labeled on the edges.
This structure satisfies the following \emph{invariants}: for all $i\in
dom(s)$, $(1)$ the nodes $(X^{in}, i)$ and $(X^{out}, i)$ exist only if
$(X,i)$ is useful, and $(2)$ there is a directed path from $(X^{in}, i)$ to $(X^{out}, i)$ whose
sequence of labels is equal to the value of the variable $X$ computed by $T$ after reading $s[i]$. 


The condition on usefulness of nodes implies that \sst-output structures consist of a single directed component, and 
therefore they are edge-labeled string structures. 
%\begin{figure}[h]
%  \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm, semithick]
 % \tikzstyle{every state}=[fill=blue!20!white,minimum size=2em]
% \node[initial, initial text={},state,fill=blue!20!white] at (0,0) (A) {q} ;
% \node[state, accepting, fill=blue!20!white] at (5,0) (B) {r} ;
% \path(B) edge  [bend right=10] node[anchor=south,above]{$a\left|\begin{array}{llllllll}X:=X\\Y:=eYf\\Z:=Z\end{array}\right.$} (A);
% \path(A) edge  [loop above] node[anchor=south,above]{$a\left|\begin{array}{llllllll}X:=aXb\\Y:=aaa\\Z:=Zc\end{array}\right.$} (A);
%   \path(A) edge [bend right=10] node[anchor=north,below]  {$b\left|\begin{array}{llllllll}X:=c\\Y:=Y\\Z:=dZc\end{array}\right.$} (B);
% \path(B) edge  [loop above] node[anchor=south,above]{$b\left|\begin{array}{llllllll}X:=X\\Y:=YbZc\\Z:=g\end{array}\right.$} (B);
%    \node[draw=none] at (-2,0) {$T_1:$};
%   \end{tikzpicture}
% \caption{An SST with Muller set $\{2\}$ and $F(\{2\})=XY$.}
% \label{mull-1}
%\end{figure}

\input{outputgraph}


As an example of \sst-output structure consider Fig. \ref{fig:outputgraph}. 
We show only the variable updates. 
 Dashed arrows represent variable updates for useless variables, and therefore does not belong the \sst-output
structure. Initially the variable content of $Z$ is equal to $\epsilon$. 
It is represented by the $\epsilon$-edge from $(Z^{in}, 0)$ to $(Z^{out}, 0)$ in the first column. 
Then, variable $Z$ is updated to $Zc$. 
Therefore, the new content of $Z$ starts with $\epsilon$ (represented by the $\epsilon$-edge from $(Z^{in},1)$ to $(Z^{in},0)$,
which is concatenated with the previous content of $Z$, and then concatenated with $c$ (it is represented by the $c$-edge from
$(Z^{out},0)$ to $(Z^{out},1)$). 
Note that the invariant is satisfied. The content of variable $X$ at position 5 is given by  
the label of the path from $(X^{in},5)$ to $(X^{out},5)$, which is 
$c$. Also note that some edges are labelled by strings with several letters, but there are finitely many possible such strings. 
In particular, we denote by $O_T$ the set of all strings that appear in right-hand side of variable updates. 
\sst-output structures are defined formally in Appendix \ref{app:sst-output}. 


We next show that the transformation that maps an $\omega$-string $s$ into its output structure 
is FO-definable, whenever the SST is 1-bounded and aperiodic. Using the fact that variable flow is FO-definable,
we show that for any two variables $X,Y$, we can capture in FO, a path from $(X^d, i)$ to $(Y^e, j)$ 
  for $d, e\in \{in, out\}$ in $G_T(s)$ and all positions $i, j$.
 We are in state $q_i$ at position $i$.  For example, there is a path
   from $(X^{in},3)$ to $(Z^{in},1)$ in Figure \ref{fig:outputgraph}. However, $Z$ at position 1 does not flow into 
   $X$ at position 3. Note that this is because of the update $X:=XY$ at position 6, and 
   $Z$ at position 1 flows into $Y$ at position 5, 
  and $X$ at position 3 flows into $X$ at position 5, and $X$ and $Y$ are catenated in order 
  at position 5 to define $X$ at position 6. Similarly, there is a path from $(Z^{d},1)$ to $(Y^{out},5)$ for $d \in \{in,out\}$.  
  This is because $Z$ at position 1 flows into $Z$ at position 4, and 
  this value of $Z$ is used in updating $Y$ at position 5 as $Y:=bZc$. Lastly, 
  there is a path  from $(Y^{in},5)$ to $(Z^{d},2)$. This is because $Z$ at position 2 
  flows into $Y$ at position 5 by the update $Y:=YbZc$. Thus, the SST output graphs have a nice property,
  which connects a path from $(X^d,i)$ to $(Y^{d'},j)$ based on the variable flow, and the catenation of variables 
  in updates. Formally, let $T$ be an \textbf{aperiodic,1-bounded} \sst{} $T$. 
    Let $s\in dom(T)$, $G_T(s)$ its \sst-output structure and $r=q_0\dots q_n\dots$ the accepting run of $T$ on $s$. 
    For all variables $X,Y\in \varsst$, all positions $i,j\in \dom(s)\cup\{0\}$, all $d,d'\in\{in,out\}$, there exists a path from node 
    $(X^{d},i)$ to node $(Y^{d'},j)$ in $G_T(s)$ iff $(X,i)$ and
    $(Y,j)$ are both useful and one of the following conditions hold: either
    \begin{enumerate}
      \item
$(q_j,Y)\flows^{s[j{+}1{:}i]}_1(q_i,X)$ and $d = in$, or
    \item 
$(q_i,X)\flows^{s[i{+}1{:}j]}_1 (q_j,Y)$ and $d' = out$, or
    \item 
there exists $k\geq max(i,j)$ and two variables $X',Y'$ such
      $(q_i,X)\flows^{s[i{{+}1:}k]}_1 (q_k,X')$, $(q_j,Y)\flows^{s[j{+}1{:}k]}_1 (q_k,Y')$
      and $X'$ and $Y'$ are concatenated in this order\footnote{by concatenated we
        mean that there exists a variable update whose rhs is of the
        form $\dots X'\dots Y'\dots$} by $r$ when reading $s[k+1]$. 
    \end{enumerate}
   Using the fact that variable flow is FO-definable, we have 
 \begin{lemma}\label{lem:fopath}
    Let $T$ be an \textbf{aperiodic,1-bounded} \sst{} $T$. 
    For all $X,Y\in \varsst$ and all $d,d'\in
    \{in,out\}$, there exists an FO[$\Sigma$]-formula 
    $\text{path}_{X,Y,d,d'}(x,y)$ with two free variables
    such that for all strings $s\in\dom(T)$ and all positions
    $i,j\in dom(s)$, $s\models \text{path}_{X,Y,d,d'}(i,j)$ iff 
    there exists a path from $(X^d,i)$ to $(Y^{d'},j)$ in
    $G_T(s)$.
\end{lemma}
The proof of Lemma \ref{lem:fopath} is in Appendix \ref{app:fopath}. 
We can now formally construct an FOT given the 1-bounded, aperiodic, SST. 
The sequence of variable substitutions of an aperiodic, 1-bounded SST over a string can be represented as the copy set 
in FOTs. As seen in Appendix (in Proposition \ref{prop:fostates}) one can write a formula 
$\phi_q(x)$ to capture the state $q$ reached in an accepting run after reading a prefix. 
For each variable $X \in \mathcal{X}$, we have two copies $X^{in}$ and $X^{out}$ that serve as the copy set 
of the FOT. As given by the SST output-structure, for each step $i$, state $q$ and symbol $a$, 
a copy is connected to copies in the previous step based on the updates $\rho(q,a)$. 
In the following, we detail this in FO. Lemma \ref{lem:fopath} then captures a path in the FOT. 
The full details of the FOT construction can be found in Appendix \ref{app-fot-cons}.
  
\end{proof}

 



